A cryptographic approach to black box adversarial machine learning

We propose a new randomized ensemble technique with a provable security guarantee against black-box transfer attacks. Our proof constructs a new security problem for random binary classifiers which is easier to empirically verify and a reduction from the security of this new model to the security of the ensemble classifier. We provide experimental evidence of the security of our random binary classifiers, as well as empirical results of the adversarial accuracy of the overall ensemble to black-box attacks. Our construction crucially leverages hidden randomness in the multiclass-to-binary reduction.

==> discussion.tex <==
These experiments demonstrate that random ensembles are a promising approach to security against black-box transfer attacks. The security of our scheme can be more reliably estimated than traditional constructions against this particular class of attacks. One important item to note is that the random ensemble construction is not compatible with standard techniques of robust training. Robust training tends to decrease the standard test error of the classifier, which means that a larger threshold $r$ needs to be used to account for natural errors in the individual random classifiers. However, a larger $r$ value leads to weaker security in the ensemble. 

%We proposed a novel approach to provable robustness at test time in the adversarial setting. We formalized a smaller attack problem which is easier to study and which we conjecture to be hard. We also show that our overall ensemble construction enjoys high adversarial accuracy against black-box attacks with standard measures of perturbation size while being completely agnostic of these parameters. Our formal proof framework introduces some techniques in analysis of cryptographic constructions to the adversarial learning problem, and we hope it can lead to more principled empirical and theoretical work in this area. 
